Seeing Your Speech Style: A Novel Zero-Shot Identity-Disentanglement Face-based Voice Conversion

Face-based Voice Conversion (FVC) is a novel task that leverages facial images to generate the target speaker's voice style. Previous work has two shortcomings: (1) suffering from obtaining facial embeddings that are well-aligned with the speaker's voice identity information, and (2) inadequacy in decoupling content and speaker identity information from the audio input. To address these issues, we present a novel FVC method, Identity-Disentanglement Face-based Voice Conversion (ID-FaceVC), which overcomes the above two limitations. More precisely, we propose an Identity-Aware Query-based Contrastive Learning (IAQ-CL) module to extract speaker-specific facial features, and a Mutual Information-based Dual Decoupling (MIDD) module to purify content features from audio, ensuring clear and high-quality voice conversion. Besides, unlike prior works, our method can accept either audio or text inputs, offering controllable speech generation with adjustable emotional tone and speed. Extensive experiments demonstrate that ID-FaceVC achieves state-of-the-art performance across various metrics, with qualitative and user study results confirming its effectiveness in naturalness, similarity, and diversity. Project website with audio samples and code can be found at https://id-facevc.github.io.

==> sec/6_checklist.tex <==
\section{Reproducibility Checklist}
\label{sec:Reproducibility Checklist}

%Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

\noindent This paper:

\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) \answerYes{yes}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) \answerYes{yes}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) \answerYes{yes}
\end{itemize}

\noindent Does this paper make theoretical contributions? (yes/no) \answerNo{no}

\noindent If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes/no) \answerYes{yes}

\noindent If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) \answerYes{yes}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) \answerNA{NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) \answerNA{NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) \answerYes{yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) \answerYes{yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \answerNA{NA}
\end{itemize}

\noindent Does this paper include computational experiments? (yes/no) \answerYes{yes}

\noindent If yes, please complete the list below.

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no). \answerNo{No, we will release the code upon publication of the paper.}
%\answerNo{No, but we provide a detailed explanation in the corresponding parts of Method and Implementation Details. Additionally, the relevant source code will be included in the released project.}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) \answerNo{No, we will release the code upon publication of the paper.}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \answerYes{yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \answerYes{yes}
%\answerPartial{partial, we will provide an explanation of the source and the meaning of the code in the released version.}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \answerYes{yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \answerPartial{Partial, but our work does not have stringent requirements for computational resources and memory; the code can be trained with just a single A40 GPU.}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \answerYes{yes}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \answerNo{No, but we ensured the robustness of our results by running preliminary tests multiple times.}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) \answerYes{yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) \answerPartial{Partial, we have used confidence intervals for subjective evaluation metrics.}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) \answerPartial{Partial, our work provides an explanation for all important parameters; others not mentioned will be reflected in the code.}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) \answerNo{No. Our paper does not explicitly state the number and range of values tried for each (hyper-) parameter during development. Instead, we relied on a combination of domain knowledge and iterative testing to select the final parameter settings.}
\end{itemize}
